Multidimensional Item Response Theory in the Style of Collaborative Filtering

This paper presents a machine learning approach to multidimensional item response theory (MIRT), a class of latent factor models that can be used to model and predict student performance from observed assessment data. Inspired by collaborative filtering, we define a general class of models that includes many MIRT models. We discuss the use of penalized joint maximum likelihood (JML) to estimate individual models and cross-validation to select the best performing model. This model evaluation process can be optimized using batching techniques, such that even sparse large-scale data can be analyzed efficiently. We illustrate our approach with simulated and real data, including an example from a massive open online course (MOOC). The high-dimensional model fit to this large and sparse dataset does not lend itself well to traditional methods of factor interpretation. By analogy to recommender-system applications, we propose an alternative "validation" of the factor model, using auxiliary information about the popularity of items consulted during an open-book exam in the course.

==> notations.tex <==
\begin{center}
\begin{tabular}{ll} \toprule
  Symbol & Description\\ \midrule
  $m$ & number of users\\
  $n$ & number of items\\
  $r$ & number of true latent dimensions\\
  $d$ & number of estimated latent dimensions\\
  $N_f$ & number of folds\\ \midrule
  $\bm{U} = (u_{ij})$ & $n \times m$ user response matrix, interactions\\
  $\bm{\Theta} = (\bm\theta_i)_{1 \leq i \leq m}$ & $m \times r$ user latent factor matrix\\
  $\bm{X} = (\bm{x}_j)_{1 \leq j \leq n}$ & item latent factor matrix\\
  $\bm\zeta$ & all parameters\\
  $z_{ij}$ & logit\\
  $p_{ij}$ & probability\\
  $\lambda, \lambda_1, \lambda_2$ & regularization parameters\\ \bottomrule
\end{tabular}
\end{center}


==> results.tex <==
%\documentclass{standalone}
%\usepackage{booktabs,multirow,multicol,unicode-math}

%\begin{document}
%\scriptsize
\begin{tabular}{llllllllllllll} \toprule
Data	& Spars.	& \multicolumn{4}{l}{Constrained JMLE}	& \multicolumn{4}{l}{Ours non regularized}				& \multicolumn{4}{l}{Ours regularized}\\
& & \multicolumn{4}{l}{\cite{chen2019joint}} & \multicolumn{4}{l}{2 batches} & \multicolumn{4}{l}{$\lambda = 0.02$, 10 batches}\\
	&	& LL	& Acc	& AUC	& Time	& LL	& Acc	& AUC	& Time	& LL	& Acc	& AUC	& Time\\ \midrule
Simulated 3 & 0\% & -24085 & 0.79 & 0.87 & & \bf -22530 & 0.81 & 0.89\\
1000 persons\\
$\times$ 60 items\\
\\
Simulated 5	& 0\% 	& -354	& 0.91	& 0.97	& 	& \bf -244	& 0.95	& 0.98\\
80 persons & 20\% 	& -205	& 0.94	& 0.99	& 	& \bf -76	& 0.98	& 1\\
$\times$ 20 items & 80\% 	& -1.11	& 1	& 1	&	& \bf -0.02	& 1	& 1\\
\\
Simulated 5	& 0\% 	& -18187	& 0.83	& 0.92	& 	& \bf -17777	& 0.83	& 0.92\\
1000 persons	& 20\% 	& -13189	& 0.85	& 0.93	& 	& \bf -12880	& 0.85	& 0.93\\
$\times$ 50 items	& 80\% 	& -1276	& 0.95	& 0.99	& 	& \bf -491	& 0.98	& 1\\
\\																
FCI Train	& 0.2\% & -116369	& 0.84	& 0.93	& $57''$	& \bf -113792	& 0.84	& 0.93	& $42''$	& -140406	& 0.82 & 0.91	& $12''$\\
FCI Test	 	&	& -31181	& 0.74	& 0.76	& 	& -49723	& 0.73	& 0.75	& 	& \bf -21461	& 0.75	& 0.77\\
\\																
MOOC Train & 64\%	& -773746	& 0.79	& 0.88	& $33'18''$	& \bf -771703	& 0.79	& 0.88	& $5'12''$ & -843627 & 0.79 & 0.86 & $2'58''$\\
MOOC Test &	& -108280	& 0.74	& 0.79	& 	& -109805	& 0.74	& 0.8 & & \bf -104761 & 0.74 & 0.80\\ \bottomrule
% FCI: 13253 x 30
% MOOC: 29294 x 197
\end{tabular}
%\end{document}

